Seeking Anonymity in an Internet Panopticon

Obtaining and maintaining anonymity on the Internet is challenging. The state of the art in deployed tools, such as Tor, uses onion routing (OR) to relay encrypted connections on a detour passing through randomly chosen relays scattered around the Internet. Unfortunately, OR is known to be vulnerable at least in principle to several classes of attacks for which no solution is known or believed to be forthcoming soon. Current approaches to anonymity also appear unable to offer accurate, principled measurement of the level or quality of anonymity a user might obtain. Toward this end, we offer a high-level view of the Dissent project, the first systematic effort to build a practical anonymity system based purely on foundations that offer measurable and formally provable anonymity properties. Dissent builds on two key pre-existing primitives - verifiable shuffles and dining cryptographers - but for the first time shows how to scale such techniques to offer measurable anonymity guarantees to thousands of participants. Further, Dissent represents the first anonymity system designed from the ground up to incorporate some systematic countermeasure for each of the major classes of known vulnerabilities in existing approaches, including global traffic analysis, active attacks, and intersection attacks. Finally, because no anonymity protocol alone can address risks such as software exploits or accidental self-identification, we introduce WiNon, an experimental operating system architecture to harden the uses of anonymity tools such as Tor and Dissent against such attacks.

==> motiv.tex <==
\section{Motivation: Why Anonymity?}

\baf{	My very old notes, delete when we decide they're no longer useful:
And what kinds of privacy do we need.

Why anonymity is fundamental to anti-tracking and hence
to online privacy in a broad sense.

Anonymity vs private communication

do only people with "something to hide" need anonymity?
- sensitive information isn't just what you're "trying to hide"
- useful against you in malicious ways, identity theft, etc
- example: recent social engineering attacks via Amazon account, etc.

collected data is not really safe from the wrong people
- internal misuse of NSA data, etc.
- historical precedent for govt use surveillance to suppress minority
	(e.g., Martin Luther King Jr)
- longevity: if it's collected now, it'll still be there in 20 years,
	who knows who'll be in office then

tracking and anti-tracking
- targeted advertising, etc.
- ability for companies to aggregate data from users
	across many different accounts, services
- federated logins
- do you know what they know about you?
- risks of stalking
}%baf

As computers and networks have become essential tools in business, government,
recreation, and many other aspects of daily life, close attention has been paid
to online privacy.  Often, the notion of ``privacy'' under consideration is
{\it confidentiality}: how to prevent unauthorized parties from accessing
sensitive information and, in particular, how to ensure that traffic can flow
over open networks but ultimately be read only by its intended recipients.  In
this paper, we address a different aspect of online privacy, namely {\it
anonymity}; how to prevent an adversary from learning who is communicating with
whom rather than what is being communicated.  Anonymous communication can be a
life-saving tool for soldiers or spies operating in hostile environments and
for political dissidents acting in opposition to repressive governments.  It
gives potential business partners the ability to communicate without their
competitors knowing that they are doing so, and it allows police officers and
prosecutors to contact witnesses and informants without revealing their identities
to criminals.  Hiding {\it patterns} of communication is in fact every bit as
important as hiding {\it contents} of communications, but it has not received
as much attention from the computer-science community until recently.

Although it is often high-stakes use cases of this sort (battlefield
communication, political dissent, {\it etc.}) that are offered as motivation
for the study of anonymous-communication technologies, anonymous activity is in
fact quite common in everyday life.  For example, paying with cash in
brick-and-mortar stores, browsing printed material in a brick-and-mortar
library, calling law-enforcement ``tip'' lines, voting, and opinion polling are
usually done anonymously.  As more and more of everyday life moves online,
people naturally want to continue to perform these tasks anonymously and, more
generally, to be free to reach out to new people and explore unconventional
paths in life without having to identify themselves.  The study of basic
anonymous-communication protocols is thus well motivated by the needs of
ordinary people, not only those of soldiers, spies, and dissidents.

\baf{	Experimentalism and fostering low-risk creativity?
	examples: 4chan, slashdot communities;
	JK Rowling's use of pseudonym on non-Harry Potter novel.}

Indeed, recent events have raised the stakes enormously in the quest for widely
accessible, easy-to-use, strong anonymity technology.  The documents leaked by
Edward Snowden have revealed that the US government is conducting warrantless
surveillance on a massive scale and, in particular, that the long-term goal of
the National Security Agency (NSA) is to be ``able to collect virtually
everything available in the digital world''~\cite{risen13nsa}.  To the
specific questions of who calls whom, when, where, and for how long, the NSA
apparently already has comprehensive answers about callers in the US,
because major US telecommunications companies have been providing this
information to the agency for years~\cite{}.  Moreover, courts have ruled
that the government does not need warrants to collect these ``metadata'' about
US persons' communications~\cite{}; warrants are still required for the
collection of ``data,'' {\it i.e.}, {\it what} is being said as opposed to who
is saying it to whom, but enforcement of even this requirement has been lax~\cite{gellman13broke}.  Unless and until there is action by the US Congress or the
courts to change this state of affairs, purely technological solutions are our
only recourse if we wish to avoid revealing all of our communication patterns
to the government. 

\com{ 
Although the word ``anonymous'' is used often in common parlance, defining it
precisely and developing network protocols that guarantee it has proven to be
quite difficult; this paper presents the basic tenets of
anonymous-communication protocols at a level suitable for non-specialists.  In
Section~\ref{sec-onion}, we consider onion routing, the most highly developed
approach to anonymity, and deployed protocols that implement it.
Section~\ref{sec-attacks} presents several known attacks on onion-routing
systems for which there are no satisfactory defenses.  In
Section~\ref{sec-dissent}, we introduce Dissent, a promising but not yet
deployed anonymous-communication system that is not based on onion routing and
hence not vulnerable to all of the same attacks.  We conclude with open
questions in Section~\ref{sec-open}.

Note that we are concerned herein {\it only} with anonymity, {\it i.e.}, with
preventing an adversary from determining who is communicating with whom.  See
[Feigenbaum2011] and the references therein for a discussion of {\it
confidentiality}, {\it unobservability}, {\it unblockability}, and other
security notions that are related to but distinct from anonymity.

References

[Chaum1981] D. Chaum, ``Untraceable Electronic Mail, Return Addresses, and Digital Pseudonyms,'' {\it Communications of the ACM}, {\bf 1:1} (1981), pp. 84-88.

[Chaum1985] D. Chaum, ``Security without Identification: Transaction Systems to make Big Brother Obsolete,'' {\it Communications of the ACM} {\bf 28:10} (1985), pp. 1030-1044.

[Chaum1986] D. Chaum, ``The Dining Cryptographers Problem: Unconditional Sender and Recipient Untraceability,'' {\it Journal of Cryptology} {\bf 1:1} (1988), pp. 65-75.

[Feigenbaum2011]  J. Feigenbaum, ``Defining `Anonymity' in Networked Communication," Technical Report YALEU/DCS/TR-1448, Yale University, New Haven CT, December 2011.

[Gellman2013] B. Gellman, ``NSA broke privacy rules thousands of times per year, audit find,'' {\it The Washington Post}, August 16, 2013.

[MyersTimmons2011] S. Myers and H. Timmons, ``Clinton Urges Countries not to Stifle Online Voices,'' {\it The New York Times}, December 8, 2011.  

[RisenPoitras2013] J. Risen and L. Poitras, ``N.S.A. Report Outlined Goals for More Power,'' {\it The New York Times}, November 22, 2013.

[Tor] Tor: Anonymity online, \url{https://www.torproject.org/}

}%com


